A computational framework for connection matrix theory

The connection matrix is a powerful algebraic topological tool from Conley index theory that captures relationships between isolated invariant sets. Conley index theory is a topological generalization of Morse theory in which the connection matrix subsumes the role of the Morse boundary operator. Over the last few decades, the ideas of Conley have been cast into a purely computational form. In this paper we introduce a computational, categorical framework for the connection matrix theory. This contribution transforms the computational Conley theory into a computational homological theory for dynamical systems. More specifically, within this paper we have two goals: 1) We cast the connection matrix theory into appropriate categorical, homotopy-theoretic language. We identify objects of the appropriate categories which correspond to connection matrices and may be computed within the computational Conley theory paradigm by using the technique of reductions. 2) We describe an algorithm for this computation based on algebraic-discrete Morse theory.

==> correctm.tex <==
% This file defines a few macros useful in team work on a paper or a book.
% The main purpose of the macros is to faciliate having simultanously two versions
% of selected fragments of text (old and new) with appropriate comments so that
% co-authors may think before deciding which version is better.
%
% To use these macros you must put this file in the directory where you keep
% the source files and add the following two lines
%
%\include{correctm}
%\showcomments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% at the beginnig of the main source file.
% If you want to compile the source file without any comments,
% just replace \showcomments by \hidecomments. In this case only the new versions
% will be used in the compiled text and all comments will be ommitted.
% This gives a possibility of looking at the clean text while still keeping
% the alternatives in the source file
%
% The \corrl macro
% ================
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The main macro is \corrl and it has the following syntax
%
% \corrl comment<<old_version||new_version>>
%
% Note that <<, || and >> are obligatory even if old_version or new_version are empty texts.
% The words 'comment', 'old_version', 'new_version',
% mark the places where you put your own text, i.e. these are parameters of the macro.
% The meaning of the parameters is
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%     'comment'     - just a comment set in a non-standard font so that it clearly differs from
%                      the proper text
%     'old_version' - here you put the old text, which you want replaced with the new text
%     'new_version' - here you put the new text
%
% If comments are turned on by \showcomments, you will see the comment, then the old version
% clearly seperated form the new version and a margin mark. If comments are turned off, you
% will see only the new version with no comments or marks.
%
% If comment, old_version and/or new_version are longer than one line, a good idea is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% to write this macro (as well as the following macros) as
% \corrl
%   comment
% <<
%   old_version
% ||
%   new_version
% >>
%
%
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% The \corrq macro
% ================
%
% Another possibility is that you feel some fragment should be changed but you do not know what
% should be the new version. Then use the macro
%
%  \corrq comment<<questioned_text>>
%
% With comments turned on you will see the comment followed by the clearly marked
% questioned text
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% The \corre macro
% ================
%
% Sometimes the new version is an almost obvious change, so you
% want the old version only in the source
% file (just in case ...) but not in the compiled file.
% Then use the macro
%
% \corre comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which in the compiled file shows only the new version and the margin mark to indicate that
% changes were made.
%
% The \corrs macro
% ================
%
% When the change is almost obvious and short, use the macro
%
% \corrs comment<<old_version||new_version>>
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%
% which is similar to the previous but automaticallly adds a comment
% old_version->new_version on the margin
%
% The \corrn and \corro macros
% ============================
%
% To settle matters you can use two more macros with the same syntax as \corrl
%
%  \corro - to force the old version - the new version and all comments are disregarded
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%                                      (but present in the source file)
%  \corrn - to force the new version - the old version and all comments are disregarded
%                                      (but present in the source file)
%
% This is simple in use (just replace l, q or s in the macro name by o or n) but leaves rubbish
% in the source file. If you find ourselve using plenty of this stuff one can easily write a simple PERL
% script which will automatically remove all this rubbish.
%
%
% The \corrc macro
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% ================
%
% This is to place in the source file a comment only. The syntax is
%
% \corrc comment <<>>
%
% Parameters containing whole paragraphs
% ======================================
%
% Note: the standard TeX macros cannot be called with parameters which go across paragraphs
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
% (i.e. contain \par or an empty line). However, there is a special mechanism which allows for that.
% It is implemented here in the form of alternative macros \longcorrl, \longcorrq, \longcorrs and so on.
% Since TeX better recovers from errors if such macros are not present, use them only when necessary.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macro definitions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\corcommstyle{\bf\tiny}
\def\corcommstyle{\bf\small\tt}

%This macro is to be used when an alternative approach is to be displayed
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%versus the old approach

\def\corrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}

{\color{red} 
 #2
 }
 
 

  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
   \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  #3
 \fi
}

\long\def\longcorrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ {\color{red}#1\marginpar{!!}}\\$<<$OLD$<<$} \end{quote}
 
 {\color{red}

  #2
  
  }
  
  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
  
    \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
  #3
  
   \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #3
 \fi
}

\def\mlabel #1
{
  \if\visiblecomments y
     \marginpar[\flushright \bf \footnotesize #1]{\bf \footnotesize #1}
  \fi
}

\def\flabel #1
{
  \if\visiblecomments y
       \hbox{\bf\footnotesize #1}
  \fi
}


%This macro is to be used when there is some confusion
%No new text is proposed

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\def\corrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill
 
 
  #2
 
  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  \noindent\hrulefill
 
\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\dotfill

  #2

  \noindent\dotfill 

\vspace{-10pt} 
 
 \noindent\hrulefill
 
 \vspace{-10pt} 
 
 \noindent\hrulefill 
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%This is just to introduce a comment

\def\corrc #1<<>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ \color{red} #1\marginpar{!!}} \end{quote}
\fi
}

%This macro is intended for some evident corrections.
%Only the new text is displayed.
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%Comment is typed on the margin.

\def\corre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
\long\def\longcorre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%This macro is intended to mark corrections to short simple typos.
%Only the new text is displayed and an automatic typo change is
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%marked on the margin.

\def\corrs #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #2 $\rightarrow$ #3\\ #1}
 \else
  #3
 \fi
}

%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%The next two macros are to help settle the matters.
%Changing \corrx where x is l,q or s to \corro (\corrn)
%will result in just choosing the old (new) text.
%This is intended to provide a simple way to get rid of
%any comments, i.e. to "clean" the paper.
%Unfortunately the no longer needed versions remain
%in the source file so in the future it would be
%useful to have some preprocessor to clean also
%the source file.
%Note that since \corrq does not provide any new stuff
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
%it makes sense only to change it to \corro unless some
%new text is added later on.

\def\corro #1<<#2||#3>>{
#2}

\def\corrn #1<<#2||#3>>{
#3}

\long\def\longcorro #1<<#2||#3>>{
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
#2}

\long\def\longcorrn #1<<#2||#3>>{
#3}

% This macro is to hide in official version pieces of text
% which is not available for presentation yet.

\long\def\underconstruction #1<<<#2>>>{
\if\visiblecomments y
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%
  \begin{quote} {\corcommstyle $<<$UNDER CONSTRUCTION - BEGIN$>>$ #1\marginpar{!!}} \end{quote}
  #2
  \begin{quote} {\corcommstyle $>>$UNDER CONSTRUCTION - END$>>$ } \end{quote}
 \else
 \fi
}



% These two macros are to tourn on/off comments
%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%

\def\showcomments{
  \let\visiblecomments y
}

\def\hidecomments{
  \let\visiblecomments n
}


%%%%%%%%%%%%%% READ ONLY VERSION %%%%%%%%%%%%%%%%


